Action in Mind: A Neural Network Approach to Action Recognition and Segmentation

Recognizing and categorizing human actions is an important task with applications in various fields such as human-robot interaction, video analysis, surveillance, video retrieval, health care system and entertainment industry. This thesis presents a novel computational approach for human action recognition through different implementations of multi-layer architectures based on artificial neural networks. Each system level development is designed to solve different aspects of the action recognition problem including online real-time processing, action segmentation and the involvement of objects. The analysis of the experimental results are illustrated and described in six articles. The proposed action recognition architecture of this thesis is composed of several processing layers including a preprocessing layer, an ordered vector representation layer and three layers of neural networks. It utilizes self-organizing neural networks such as Kohonen feature maps and growing grids as the main neural network layers. Thus the architecture presents a biological plausible approach with certain features such as topographic organization of the neurons, lateral interactions, semi-supervised learning and the ability to represent high dimensional input space in lower dimensional maps. For each level of development the system is trained with the input data consisting of consecutive 3D body postures and tested with generalized input data that the system has never met before. The experimental results of different system level developments show that the system performs well with quite high accuracy for recognizing human actions.

==> auxiliary_texfiles/datasheet.tex <==
\newcounter{aformdx}
\newcounter{aformdy}
\newcounter{aformx}
\newcounter{aformy}
\newcounter{aformtx}
\newcounter{aformtdx}
\newcounter{aformty}
\def\aformw{395}
\def\aformwhalf{\aformw / 2}
\def\aformwquart{\aformw / 4}
\def\aformwthreeq{\aformw / 4 * 3}
\def\aformh{517}
\def\aformb{23}
\def\aformlinew{0.4pt}
\def\aformrowh{20}
\def\aformRowh{27}
\newcommand\aformhline
{\put(\value{aformx},\value{aformy}){\line(1,0){\value{aformdx}}}}
\newcommand\aformvline
{\put(\value{aformx},\value{aformy}){\line(0,-1){\value{aformdy}}}}
\newcommand\aformvlinec
{\put(\value{aformx},\value{aformy}){\line(0,-1){16.25}}}
\newcommand\aformboxbase[5]
{
  \setcounter{aformtx}{\value{aformx}}
  \setcounter{aformtdx}{\value{aformdx}}
  \setcounter{aformty}{\value{aformy}}
  \addtocounter{aformtx}{#1}
  \addtocounter{aformtdx}{-#2}
  \addtocounter{aformty}{-#3}
  \put(\value{aformtx},\value{aformty})
  {
    \parbox[t]{\value{aformtdx}pt}
    {{\sf\tiny #4}{\scriptsize #5\par}}
  }
}
\newcommand\aformbox[2]{\aformboxbase{2}{11}{8}{#1}{#2}}
\newcommand\aformBox[2]{\aformboxbase{2}{11}{8}{#1}{#2}}

\begin{center}
\begin{picture}(\aformw,542)(0,0)
\linethickness{\aformlinew}
\put(0,\aformb){\framebox(\aformw,\aformh){}}
\put(-14,200){\rotatebox{90}{\parbox{200pt}
{\sf\tiny
DOKUMENTDATABLAD
enl SIS 61 41 21\\
}}}
\setcounter{aformx}{0}
\setcounter{aformy}{\aformb}
\addtocounter{aformy}{\aformh}
\setcounter{aformdx}{\aformwhalf}
\aformbox{Organization}
{\\
{\bf LUND UNIVERSITY}\vspace{0.1cm}
\\
{\myDepartment\\
\myAddress}
}
\setcounter{aformdy}{\aformrowh}
\addtocounter{aformdy}{\aformrowh}
\addtocounter{aformdy}{\aformrowh}
\addtocounter{aformdy}{\aformRowh}
\setcounter{aformx}{\aformwhalf}
\aformvline
\setcounter{aformx}{0}
\addtocounter{aformy}{-\aformrowh}
\addtocounter{aformy}{-\aformrowh}
\addtocounter{aformy}{-\aformRowh}
\aformbox{Author(s)}{\\\myName}
\setcounter{aformdy}{\aformrowh}
\aformhline
\addtocounter{aformy}{\aformrowh}
\addtocounter{aformy}{\aformrowh}
\addtocounter{aformy}{\aformRowh}
\setcounter{aformx}{\aformwhalf}
\aformbox{Document name}{\\{\bf DOCTORAL DISSERTATION}}
\addtocounter{aformy}{-\aformrowh}
\aformhline
\aformbox{Date of disputation}{\\\myFormDefenceDate}
\setcounter{aformx}{\aformwhalf}
\aformhline
\addtocounter{aformy}{-\aformrowh}
\addtocounter{aformdy}{\aformRowh}
\aformbox{Sponsoring organization}{\\Lund University Cognitive Science and the EU FET project WYSIWYD}
\aformhline
\addtocounter{aformy}{-\aformRowh}
\addtocounter{aformy}{-\aformrowh}
\setcounter{aformx}{0}
\setcounter{aformdx}{\aformw}
\aformhline
\aformbox{Title and subtitle }{\\\myTitle}
\addtocounter{aformy}{-\aformRowh}
\setcounter{aformx}{0}
\aformhline
\aformBox{Abstract}
{\\
{\parskip0pt\parindent1em
\myAbstract
}
}
\setcounter{aformy}{\aformb}
% Correspond to one minus each in the bottom section
\addtocounter{aformy}{\aformRowh}
\addtocounter{aformy}{\aformRowh}
\addtocounter{aformy}{\aformRowh}
\addtocounter{aformy}{\aformRowh}
\addtocounter{aformy}{\aformrowh}
\addtocounter{aformy}{\aformrowh}
\addtocounter{aformy}{10}
\addtocounter{aformy}{10}
\aformhline
\aformbox{Key words}
{
\\\myFormKeywords
}
\addtocounter{aformy}{-\aformRowh}
\addtocounter{aformy}{-10}
\aformhline
\aformbox{Classification system and/or index terms (if any)}{}
\addtocounter{aformy}{-\aformRowh}
\aformhline
\aformbox{Supplementary bibliographical information}{}
\setcounter{aformx}{\aformwthreeq}
\setcounter{aformdx}{\aformwquart}
\setcounter{aformdy}{\aformRowh}
\aformvline
\aformbox{Language}{\\English}
\addtocounter{aformy}{-\aformRowh}
\setcounter{aformx}{0}
\setcounter{aformdx}{\aformw}
\aformhline
\aformbox{ISSN and key title}{\\1101-8453 Lund University Cognitive Studies 172}
\setcounter{aformx}{\aformwthreeq}
\addtocounter{aformdy}{10}
\aformvline
\addtocounter{aformdy}{-10}
\aformbox{ISBN}{\\\myISBNprint\xspace(print)\\\myISBNpdf\xspace(pdf)}
\addtocounter{aformy}{-\aformRowh}
\addtocounter{aformy}{-10}
\setcounter{aformx}{0}
\aformhline
\aformbox{Recipient's notes}{}
\setcounter{aformx}{\aformwhalf}
\setcounter{aformdy}{\aformrowh}
\addtocounter{aformdy}{\aformrowh}
\aformvline
\aformbox{Number of pages}{\\\myPages}
\setcounter{aformx}{\aformwthreeq}
\aformbox{Price}{}
\setcounter{aformdy}{\aformrowh}
\aformvline
\addtocounter{aformy}{-\aformrowh}
\setcounter{aformx}{\aformwhalf}
\setcounter{aformdx}{\aformwhalf}
\aformhline
\aformbox{Security classification}{}
\setcounter{aformx}{0}
\setcounter{aformdx}{\aformw}
\addtocounter{aformy}{-\aformrowh}
\addtocounter{aformy}{-4}
\aformbox{}
{\scriptsize I, the undersigned, being the copyright owner of the abstract of the
above-mentioned dissertation, hereby grant to all reference sources
the permission to publish and disseminate the abstract of the
above-mentioned dissertation.
}
\addtocounter{aformy}{-\aformRowh}
\addtocounter{aformy}{-20}
\aformbox{
\hspace{0pt}
%\put(44,1){\includegraphics{images/signature}} %Media-Tryck does not want this to be included as a graphic
}{}
\aformbox{\rm
\scriptsize
Signature \underline{\hskip 140pt}\hfill Date \underline{\hskip 160pt}
}{}
\addtocounter{aformy}{1}
\aformbox{}{\hskip 280pt \scriptsize \myFormSignDate}
\end{picture}
\end{center}

